Fully Fine-tuned CLIP Models are Efficient Few-Shot Learners

Prompt tuning, which involves training a small set of parameters, effectively enhances the pre-trained Vision-Language Models (VLMs) to downstream tasks. However, they often come at the cost of flexibility and adaptability when the tuned models are applied to different datasets or domains. In this paper, we explore capturing the task-specific information via meticulous refinement of entire VLMs, with minimal parameter adjustments. When fine-tuning the entire VLMs for specific tasks under limited supervision, overfitting and catastrophic forgetting become the defacto factors. To mitigate these issues, we propose a framework named CLIP-CITE via designing a discriminative visual-text task, further aligning the visual-text semantics in a supervision manner, and integrating knowledge distillation techniques to preserve the gained knowledge. Extensive experimental results under few-shot learning, base-to-new generalization, domain generalization, and cross-domain generalization settings, demonstrate that our method effectively enhances the performance on specific tasks under limited supervision while preserving the versatility of the VLMs on other datasets.

==> tex/abstract.tex <==
\begin{abstract}

% \textcolor{blue}{Current prompt learning involves fine-tuning a few sets of parameters to transfer the CLIP models to downstream few-shot tasks, which often encounter the challenge of losing the model's original generalizability.

% Current Prompt-based Tuning methods equip the pre-trained Vision-Language Models (VLMs) the professionalism on specific downstream tasks but often compromise their versatility on the other datasets and domains.

% Prompt learning, which involves training only a small set of parameters, has recently become a prevalent strategy for adapting pre-trained Vision-Language Models (VLMs) to specific downstream tasks. However, while prompt-based approaches effectively endow the VLMs with enhanced performance on these tasks, they often come at the cost of reduced flexibility and adaptability when the tuned models are applied to datasets or domains other than the one they were trained on. 

Prompt tuning, which involves training a small set of parameters, effectively enhances the pre-trained Vision-Language Models (VLMs) to downstream tasks. However, they often come at the cost of flexibility and adaptability when the tuned models are applied to different datasets or domains. In this paper, we explore capturing the task-specific information via meticulous refinement of entire VLMs, with minimal parameter adjustments. When fine-tuning the entire VLMs for specific tasks under limited supervision, overfitting and catastrophic forgetting become the defacto factors. To mitigate these issues, we propose a framework named CLIP-CITE via designing a discriminative visual-text task, further aligning the visual-text semantics in a supervision manner, and integrating knowledge distillation techniques to preserve the gained knowledge. Extensive experimental results under few-shot learning, base-to-new generalization, domain generalization, and cross-domain generalization settings, demonstrate that our method effectively enhances the performance on specific tasks under limited supervision while preserving the versatility of the VLMs on other datasets.

% versatility and maintaining generalizability in limited-sample scenarios. 


% Extensive experimental results demonstrate the superiority of our method under few-shot learning, base-to-new generalization, domain generalization, and cross-domain generalization settings. Notably, our fine-tuning method performs comparable or even better than the popular prompt-based competitors, especially under the cross-domain generalization setting.

% In this paper, we focus on investigating the efficacy of full fine-tuning the pre-trained CLIP model for the downstream tasks under the limited-data scenarios. 


% \textcolor{blue}{To mitigate the overfitting, semantic conflict, and catastrophic forgetting issues that the existing fine-tuning methods often encounter, we propose to fine-tune the whole CLIP model by designing a discriminative visual-text task, further aligning the visual-text semantics in a supervision manner, and integrating knowledge distillation techniques to preserve the knowledge. }

% Extensive experimental results demonstrate the superiority of our method under few-shot learning, base-to-new generalization, domain generalization, and cross-domain generalization settings, indicating that our method enhances the CLIP's capabilities in adaptation, feature representation, and generalization in scenarios with limited data availability. It is important to note that our fine-tuning method performs comparable or even better than the popular prompt-based competitors, especially under the cross-domain generalization setting.


% Extensive experimental results demonstrate the superiority of our method under few-shot learning, base-to-new generalization, domain generalization, and cross-domain generalization settings. It is important to note that our fine-tuning method performs comparable or even better than the popular prompt-based competitors, especially under the cross-domain generalization setting.  

  


% in the limited-data regime when adapting it to downstream tasks. 
\end{abstract}

% Instead of 现在流行的prompt learning 借助少量参数在特定任务上进行微调，我们提出全量微调CLIP模型到下游少样本任务上。在数据量少的时候，全量微调很容易出现过拟合的问题，我们提出了一种CLIP-CITE的方法来加强CLIP模型的图文增强能力。为了更好泛化到下游任务上，我们提出了discriminative loss。


% feature representation

% The fine-tuning method as a common way to improve the performance of downstream tasks is not well explored and limited to the training samples and domain-of-distributions. 
% Pretrained vision-language models (VLMs) such as
% CLIP has shown impressive generalization capability in downstream vision tasks with appropriate text prompts.


% Large vision-language models have shown powerful zero-shot inference performance for downstream tasks. Fine-tuning CLIP can further improve the performance of downstream tasks. However, the standard fine-tuning methods encounter challenges that fail to work well under limited supervision and out-of-distributions. In this paper, we focus on fine-tuning CLIP to generalize to the few-shot learning and out-of-distributions downstream tasks. We propose a simple but effective framework for fine-tuning the CLIP model: Fine-Tuning with task-specific and task-agnostic objectives (FT-TSTA). Specifically, we build the classifier of downstream tasks with text-guidance features to optimize the task-specific loss \textit{i.e.} cross-entropy. To alleviate the model overfitting of the downstream data distributions and exploit the multimodal alignment knowledge in the pre-trained CLIP model, we construct a supervised vision-language contrastive learning task that fine-tunes both the text and the image encoder. Moreover, FT-TSTA utilizes a vision-language similarity distillation loss to mimic the generalized modal similarity from the CLIP model. Ultimately, FT-TSTA achieves surprisingly robust performance on the few-shot-learning, base-to-new, and out-of-distribution three benchmarks, \textit{i.e.} obtains 16.45\% gains in base-class accuracy and 2.15\% gains in new-class accuracy compared to the zero-shot CLIP model. 
